Massive Data-Centric Parallelism in the Chiplet Era

Recent works have introduced task-based parallelization schemes to accelerate graph search and sparse data-structure traversal, where some solutions scale up to thousands of processing units (PUs) on a single chip. However parallelizing these memory-intensive workloads across millions of cores requires a scalable communication scheme as well as designing a cost-efficient computing node that makes multi-node systems practical, which have not been addressed in previous research. To address these challenges, we propose a task-oriented scalable chiplet architecture for distributed execution (Tascade), a multi-node system design that we evaluate with up to 256 distributed chips -- over a million PUs. We introduce an execution model that scales to this level via proxy regions and selective cascading, which reduce overall communication and improve load balancing. In addition, package-time reconfiguration of our chiplet-based design enables creating chip products that optimized post-silicon for different target metrics, such as time-to-solution, energy, or cost. We evaluate six applications and four datasets, with several configurations and memory technologies to provide a detailed analysis of the performance, power, and cost of data-centric execution at a massive scale. Our parallelization of Breadth-First-Search with RMAT-26 across a million PUs -- the largest of the literature -- reaches 3021 GTEPS.

==> txt/TODOs.tex <==

% -The DAC cost paper could take into account area of different integrations of memory, taking Ariane as an area reference.
% 2D (cheap package), 2.5D, with or without HBM, and 3D.
% -A Python cost model. Open source with publication of this paper...
% -Evaluation? Cost of AMD Ryzen Ian cutress? Cost of Nvidia GPU. Cost of Intel Shaphire Rapids.
% -We also analyze different transistor nodes, for interposer and for 2D integration.
% -Area cost is not affected by the mask much, look at NRE for bigger dies.
% -Talk about per-wafer cost of different technologies if we tapeout 100 wafers or 100000 wafers.
% -NRE and TCO!

MICRO:
-Fix template
-Fix demonstrate based on new numbers
-Fix Proxy Figure to show

ESIN:
-reshufle background
-Proxy / cascade figure
-Approach section re-write part on proxy to reflect Figure and whatever else is neeed to explain cascading (selective)


MARCELO:
-Fix template weirdness
-Babysit jobs
-Hoist Dalorex comparison to beginning of Results
-Swap T3 latency figure with Proxy Hill (need some runs between 4 and 32)


TODO:
-Fix footnotes by adding them to the text



APPROACH:
-Explain shared-mem area! MOD X and MOD Y
-Explain cascading

EVALUATE
-Cascading feature: write through and back?
--Writeback no deadlock because it stores until writeback again
--WriteThru could be implemented as priority writeback! Or just don't do cascading
--Writeback when it's idle, and do not revisit frontier until no new tasks have been received in the last X cycles.
--Read about priority queueing University Toronto

-Proxy sizes?
-Re-run experiments

Different than Dalorex:
-Data placement? Maybe with Proxy we don't need to do low-order placement?
-Barrier to avoid useless work? Utilization still very low. Try that after the iso-distant area (give name)

DCRA changes: change title, selling narrative 
-Change Citation for dalorex
-We rethink the design of the memory system in modern processors to improve performance and energy efficiency in the context of irregular apps

MRM meeting==
Here it's a set of problems that a real system might have.
Chiplets, constrains, connectivity, loading time from disk.
Wafer scale computing is of interest. Cost is profound.
We want to use chiplets because of HBM
Tailor Design Decisions instead of configurable!
Post-tapeout, more focus there, narrative
Evaluation against Dalorex
ASPLOS better option?
-The owner delegating instead of stealing. Complications for deadlock routing if we re-send


-----------------
From the literature in graph processing, PIM-based proposals are the direct comparison with Dalorex, since they also have a memory system that scales with the amount of computing resources, and they also use ISA-programmable cores that can execute applications outside the graph domain.
From these works we compare with Tesseract~\cite{tesseract}.
We also have simulated a more recent PIM-based approach GraphQ~\cite{2019graphq} which reported 3.3$\times$ performance and 1.8$\times$ energy improvements on average over Tesseract.
However, despite communicating with the authors, we were unable to obtain the cycle and energy values from simulation outputs that matched their results.
We do not include GraphQ in our discussion because the runtime and energy consumption we reproduced were 3.2$\times$ and 4.6$\times$ bigger (geomean), respectively, compared to these publications.

We also looked at the literature in graph accelerators, i.e., those with a specialized hardware pipeline to process the different stages of graph traversing, and focused on Polygraph---the latest work.
We evaluated the code that the authors kindly provided, and experimentally confirmed that Polygraph's performance plateaus after 16 cores, while \proj{} continues to scale.
This is expected since that configuration already saturates the 512GB/s of DRAM bandwidth.

When running \proj{} with equal number of processing elements, its performance is, in geomean, within

We observed that a configuration with an equal amount of processing elements, 256, we are within \% of their performance across the same datasets we evaluated in Fig.5.
However, when we try larger configurations, they don't scale because of having saturated the memory bandwidth. When looking at both approaches with 1024 processing elements, we find that \proj{} is X$\times$ more performant.

Polygraph is not designed for scalable, but hardware acceleration.
We compare with Tesseract because it's the memory scalable solution.
We wanted to confirm our expectation, and we experimentally found that Polygraph didn't scale performance after using 256 processing elements because of being limited by DRAM BW.
For a smaller configuration using 64 processing elements (4 Polygraph cores with 16-way parallelism), we found that the performance was within a 20\% range, in geomean.

Because Poly aims at optimizing load-balance between processing elements, once BW and network resources are not constraint, we cannot directly compare with them.

2) Software programmable. Scalability of the memory system.

3) How we win
They use heuristic, decide based on data-local.

-CONCLUSION: say about reproducing results, open source repo? or say Artifact evaluation
-Mention ISA programmable in Approach
-Dalorex-full on Figure 5
-Explain how the code is split? Talk about generalized compiler passes? Like Pipette or Desc, DEC++
-Talk about how eDRAM sucks in terms of density.
+Related work with SAM&TAM
+Related work wth Execution Migration Machine (EM) MIT, Devadas

==TEXT==
-Core to scratchpad area ratio?
-Refine claims
-mention strong scaling, as a way that we can do a graph partition with many more cores
-Better explain our 2MB sweet spot

-Refactor Mesh to matrix of tiles, interconnected as a torus or a mesh
-Replace Kron with RMAT??
-Replace 'Nodes' with 'Vertices', that's how they call them at Graphit



-Lower Effective bandwidth on DRAM with irregular Apps
-Embedded DRAM? 2-8MB mem per core. Limits of parallelization? the limit is more on the chip size. At wafer scale latency also affects.
Larger graphs just use more chips.
\textbf{Limitation}: Can't do a huge graph with a single chip. You could do that with HMC, but then we aren't parallelizing as much as we could.
If the point is to execute any size with a single chip, then eDRAM (out of the scope of this paper), if the point is to execute it fast, then we can parallelize more.










==FUTURE WORK, Outside the scope of this paper==

the only way to improve is by adding special instructions to the core for graph operations, what makes it slowly become an accelerator
And then the paper would be a network of small accelerators
Works have been proposed for doing ML-friendly thin core, manycores but not as much for graph-apps friendly

-cache-duality for different operating modes on manycores.
-chiplet integration vs monolitic chip, chiplets could contain a replica, to reduce inter chiplet communication
-Two types of SRAM memory or voltage scaling with ~\cite{variable_mem}, e.g. for Edge and Node arrays.
-In-depth comparison of DRAM and SRAM power with irregular accesses?

-Implementing global barrier?
-library of apps split into dalorex code.

==SIMULATOR==
-Nicer way to count instructions -> migrate to LLVM? 
In a similar fashion as MosaicSim simulates instructions.
-Integrate into MosaicSim


## HASHING
Hash the graph instead of the processing. Low bit hashing would involve extra Route3-1 communication. We don't want to have nodes separately, because of begin end redundancy
Not give extra explanation, just assume the graph is not sorted, re-hash
Not do:
Hashing type is select-able per task! task4 to task1, no hashing? then how to send the seed? the seed could also be in software, as a variable assigned to 1 of the tiles, value 0 (root) doesn't care about hashing
Pad nodes/edges to be multiple of #cores, so that the last tile also contains as many cores. Those nodes would have no neighbors

Write a nice email to my advisor explanaing why I haven't done progress this week:

